High-resolution imaging of $Kepler$ planet host candidates. A comprehensive comparison of different techniques

The Kepler mission has discovered thousands of planet candidates. Currently, some of them have already been discarded; more than 200 have been confirmed by follow-up observations, and several hundreds have been validated. However, most of them are still awaiting for confirmation. Thus, priorities (in terms of the probability of the candidate being a real planet) must be established for subsequent observations. The motivation of this work is to provide a set of isolated (good) host candidates to be further tested by other techniques. We identify close companions of the candidates that could have contaminated the light curve of the planet host. We used the AstraLux North instrument located at the 2.2 m telescope in the Calar Alto Observatory to obtain diffraction-limited images of 174 Kepler objects of interest. The lucky-imaging technique used in this work is compared to other AO and speckle imaging observations of Kepler planet host candidates. We define a new parameter, the blended source confidence level (BSC), to assess the probability of an object to have blended non-detected eclipsing binaries capable of producing the detected transit. We find that 67.2% of the observed Kepler hosts are isolated within our detectability limits, and 32.8% have at least one visual companion at angular separations below 6 arcsec. We find close companions (below 3 arcsec) for the 17.2% of the sample. The planet properties of this sample of non-isolated hosts are revised. We report one possible S-type binary (KOI-3158). We also report three possible false positives (KOIs 1230.01, 3649.01, and 3886.01) due to the presence of close companions. The BSC parameter is calculated for all the isolated targets and compared to both the value prior to any high-resolution image and, when possible, to observations from previous high-spatial resolution surveys in the Kepler sample.

==> Table_ObsSummary.tex <==
\begin{table*}[h]
\setlength{\extrarowheight}{3pt}
\caption{\label{tab:ObsSummary} }
\centering
\begin{tabular}{lc|ccc|ccc}
\hline
\hline

Obs. Type & Instrument                   &  \multicolumn{3}{c|}{Group A}  & \multicolumn{3}{c}{Group B}\\
  & & A1 & A2 & A3 &  B1 & B2 & B3    \\ \hline
High-res. Imaging & AstraLux                 & 57 & 27 & 17 &  & & \\       
Low-res. Imaging & CAFOS                     & 20 (10)   &15  & 12 &--- & --- & ---  \\ 
Low-res. Spec. & CAFOS                          &   &  &  &--- & --- & --- \\ 


\hline
\hline

\end{tabular}
\end{table*}

==> Table_Sensitivity.tex <==
\addtocounter{table}{1}
\small
%
\longtab{4}{
\begin{longtable}{r|cccc|cccc}
\caption{ Sensitivity limits for each KOI. We show the $3-\sigma$ detection limits for angular separation 0.2\arcsec, 0.5\arcsec,1.0\arcsec,2.0\arcsec and two selection rates for the Calar Alto/AstraLux images, 5\% and 10\% (see section \S~\ref{sec:sensitivity}). \label{tab:sensitivity}  } \\

\setlength{\extrarowheight}{0.5pt}\\
\hline\hline

     KOI   &  \multicolumn{4}{c|}{5\% sel. rate}  &  \multicolumn{4}{c}{10\% sel. rate} \\
            &  $\delta=0.2$\arcsec &  $\delta=0.5$\arcsec  &  $\delta=1.0$\arcsec  &  $\delta=2.0$\arcsec  & $\delta=0.2$\arcsec  & $\delta=0.5$\arcsec  &  $\delta=1.0$\arcsec   &  $\delta=2.0$\arcsec  \\ 

\hline
\endfirsthead
\caption{continued.}\\
\hline\hline

     KOI   &  \multicolumn{4}{c|}{5\% sel. rate}  &  \multicolumn{4}{c}{10\% sel. rate} \\
            &  $\delta=0.2$\arcsec &  $\delta=0.5$\arcsec  &  $\delta=1.0$\arcsec  &  $\delta=2.0$\arcsec  & $\delta=0.2$\arcsec  & $\delta=0.5$\arcsec  &  $\delta=1.0$\arcsec   &  $\delta=2.0$\arcsec  \\ 
\hline
\endhead
\hline
\endfoot


      0012   &   1.05   &   2.11  &    4.19  &    6.84  &    1.10  &    2.06   &   4.06  &   6.89  \\
      0196   &   1.07   &   2.30  &    3.74  &    5.15  &    1.12  &    2.28   &   3.68  &   5.31  \\
      0199   &   0.96   &   2.93  &    4.82  &    5.79  &    0.96  &    2.87   &   4.83  &   6.05  \\
      0209   &   0.90   &   2.28  &    3.89  &    5.84  &    0.88  &    2.23   &   3.80  &   6.02  \\
      0211   &   1.08   &   1.74  &    3.10  &    4.14  &    1.14  &    1.71   &   3.09  &   4.38  \\
 %     0245   &   5.94   &   6.21  &    0.00  &    0.00  &    5.88  &    6.16   &   0.00  &   0.00  \\
      0330   &   1.00   &   3.13  &    5.38  &    6.78  &    0.88  &    2.87   &   5.13  &   6.96  \\
      0338   &   1.00   &   2.44  &    3.84  &    5.55  &    1.04  &    2.36   &   3.74  &   5.62  \\
      0339   &   0.93   &   2.19  &    3.83  &    5.03  &    0.91  &    2.12   &   3.78  &   5.33  \\
      0345   &   0.40   &   0.48  &    1.90  &    4.73  &    1.67  &    2.08   &   2.33  &   3.15  \\
      0349   &   0.89   &   2.45  &    4.72  &    6.34  &    0.92  &    2.35   &   4.71  &   6.59  \\
      0351   &   1.27   &   2.15  &    3.37  &    5.12  &    1.28  &    2.13   &   3.37  &   5.32  \\
      0366   &   0.90   &   2.48  &    4.10  &    6.39  &    0.88  &    2.44   &   4.00  &   6.40  \\
 %     0385   &   0.47   &   0.00  &    0.00  &    0.00  &    0.72  &    0.28   &   1.82  &   4.89  \\
      0386   &   1.13   &   2.19  &    3.63  &    5.44  &    1.20  &    2.17   &   3.57  &   5.61  \\
      0388   &   1.20   &   2.38  &    3.60  &    5.55  &    1.20  &    2.33   &   3.55  &   5.60  \\
      0393   &   0.94   &   2.18  &    4.29  &    5.54  &    0.97  &    2.13   &   4.22  &   5.77  \\
      0408   &   1.53   &   1.72  &    2.40  &    3.43  &    1.60  &    1.79   &   2.47  &   3.78  \\
      0416   &   0.96   &   2.19  &    3.45  &    5.68  &    0.96  &    2.14   &   3.37  &   5.73  \\
      0422   &   1.00   &   1.94  &    3.34  &    4.85  &    1.04  &    1.91   &   3.32  &   5.10  \\
      0431   &   1.12   &   2.54  &    4.13  &    5.62  &    1.12  &    2.47   &   4.08  &   5.83  \\
      0463   &   1.10   &   2.50  &    3.92  &    5.58  &    1.10  &    2.43   &   3.86  &   5.78  \\
      0473   &   1.23   &   1.71  &    2.74  &    3.98  &    1.31  &    1.71   &   2.68  &   4.23  \\
      0478   &   0.97   &   2.36  &    4.19  &    5.85  &    1.00  &    2.31   &   4.12  &   6.04  \\
      0481   &   1.12   &   1.64  &    2.92  &    4.02  &    1.19  &    1.66   &   2.92  &   4.23  \\
%      0490   &   0.43   &   0.41  &    1.79  &    4.54  &    1.73  &    1.87   &   2.32  &   3.82  \\
      0496   &   0.91   &   2.20  &    3.55  &    5.64  &    0.95  &    2.17   &   3.51  &   5.78  \\
      0524   &   1.22   &   1.78  &    2.93  &    4.09  &    1.27  &    1.76   &   2.88  &   4.36  \\
      0528   &   1.40   &   1.77  &    2.80  &    3.87  &    1.42  &    1.83   &   2.85  &   4.16  \\
      0534   &   1.07   &   2.60  &    4.26  &    5.46  &    1.12  &    2.52   &   4.23  &   5.67  \\
      0561   &   1.12   &   2.12  &    3.15  &    5.14  &    1.13  &    2.08   &   3.08  &   5.27  \\
      0567   &   1.00   &   2.11  &    4.12  &    5.66  &    1.09  &    2.13   &   3.96  &   5.86  \\
      0568   &   1.20   &   2.63  &    4.17  &    5.62  &    1.30  &    2.60   &   4.11  &   5.84  \\
      0571   &   1.12   &   1.60  &    3.09  &    4.34  &    1.18  &    1.60   &   3.05  &   4.59  \\
      0579   &   0.96   &   2.86  &    4.96  &    6.53  &    0.96  &    2.80   &   4.91  &   6.78  \\
      0589   &   0.96   &   3.28  &    5.77  &    6.34  &    0.96  &    3.20   &   5.88  &   6.61  \\
      0617   &   1.10   &   2.56  &    4.44  &    5.51  &    1.10  &    2.48   &   4.40  &   5.79  \\
      0625   &   1.00   &   2.50  &    4.70  &    5.94  &    1.00  &    2.45   &   4.70  &   6.18  \\
      0632   &   0.93   &   2.75  &    4.69  &    6.76  &    0.93  &    2.60   &   4.58  &   6.96  \\
      0654   &   1.07   &   2.40  &    4.53  &    5.57  &    1.07  &    2.33   &   4.46  &   5.84  \\
      0659   &   0.93   &   2.87  &    5.44  &    6.98  &    0.91  &    2.80   &   5.37  &   7.25  \\
      0664   &   0.90   &   3.09  &    5.23  &    6.98  &    0.90  &    3.03   &   5.17  &   7.18  \\
      0671   &   0.96   &   2.18  &    4.45  &    6.18  &    1.00  &    2.09   &   4.36  &   6.38  \\
      0676   &   1.04   &   2.40  &    4.18  &    6.22  &    1.04  &    2.34   &   4.04  &   6.44  \\
      0678   &   0.96   &   2.40  &    4.28  &    6.44  &    1.00  &    2.31   &   4.14  &   6.63  \\
      0684   &   1.00   &   2.60  &    5.07  &    5.95  &    1.00  &    2.55   &   5.08  &   6.22  \\
      0686   &   1.00   &   2.53  &    4.80  &    6.12  &    1.00  &    2.45   &   4.76  &   6.40  \\
      0693   &   1.04   &   2.74  &    5.13  &    6.24  &    1.04  &    2.65   &   5.10  &   6.49  \\
      0695   &   1.28   &   2.22  &    3.23  &    4.94  &    1.30  &    2.21   &   3.18  &   5.05  \\
      0709   &   1.00   &   3.07  &    5.68  &    6.65  &    1.00  &    2.93   &   5.65  &   6.91  \\
      0717   &   0.88   &   2.80  &    5.11  &    6.97  &    0.87  &    2.74   &   5.06  &   7.15  \\
      0739   &   1.20   &   2.60  &    4.06  &    4.88  &    1.20  &    2.55   &   4.07  &   5.14  \\
      0884   &   1.23   &   1.74  &    3.12  &    3.99  &    1.30  &    1.75   &   3.17  &   4.27  \\
      1015   &   1.36   &   2.90  &    4.09  &    5.28  &    1.36  &    2.88   &   4.06  &   5.53  \\
      1236   &   1.20   &   2.24  &    3.45  &    5.23  &    1.20  &    2.22   &   3.37  &   5.46  \\
      1268   &   1.12   &   2.43  &    3.82  &    5.24  &    1.20  &    2.40   &   3.81  &   5.44  \\
      1326   &   1.40   &   2.91  &    3.15  &    3.81  &    1.60  &    3.08   &   3.34  &   4.08  \\
      1353   &   0.96   &   2.55  &    5.03  &    6.23  &    0.96  &    2.49   &   4.94  &   6.47  \\
      1376   &   1.33   &   2.58  &    3.60  &    4.98  &    1.33  &    2.58   &   3.58  &   5.20  \\
      1426   &   0.96   &   2.44  &    4.18  &    5.83  &    0.96  &    2.36   &   4.11  &   6.06  \\
      1452   &   1.00   &   2.53  &    4.91  &    6.19  &    1.04  &    2.44   &   4.80  &   6.43  \\
      1529   &   1.21   &   1.72  &    3.04  &    3.74  &    1.30  &    1.73   &   3.08  &   4.03  \\
      1596   &   1.11   &   1.83  &    3.36  &    4.12  &    1.22  &    1.83   &   3.36  &   4.40  \\
      1684   &   1.04   &   2.30  &    4.17  &    6.40  &    1.07  &    2.27   &   4.05  &   6.54  \\
      1701   &   0.93   &   2.57  &    5.05  &    6.98  &    0.93  &    2.50   &   4.97  &   7.14  \\
      1779   &   1.00   &   2.50  &    4.64  &    6.55  &    1.00  &    2.44   &   4.55  &   6.67  \\
      1800   &   1.12   &   2.43  &    4.15  &    6.36  &    1.12  &    2.37   &   4.03  &   6.49  \\
      1894   &   0.96   &   2.65  &    4.85  &    6.91  &    0.93  &    2.55   &   4.76  &   7.07  \\
%      1924   &   6.68   &   6.87  &    0.00  &    0.00  &    6.30  &    6.53   &   0.00  &   0.00  \\
%      1925   &   6.98   &   7.12  &    0.00  &    0.00  &    6.83  &    7.00   &   0.00  &   0.00  \\
      2042   &   1.07   &   2.33  &    4.32  &    6.35  &    1.07  &    2.28   &   4.19  &   6.49  \\
      2124   &   1.20   &   2.45  &    3.06  &    4.07  &    1.20  &    2.54   &   3.12  &   4.32  \\
      2133   &   1.04   &   2.71  &    4.88  &    7.18  &    0.96  &    2.48   &   4.57  &   7.20  \\
      2260   &   0.93   &   2.69  &    5.39  &    6.80  &    0.93  &    2.63   &   5.30  &   7.00  \\
      2324   &   1.04   &   2.49  &    4.59  &    6.38  &    1.04  &    2.44   &   4.45  &   6.48  \\
      2352   &   6.50   &   6.73  &    0.00  &    0.00  &    6.38  &    6.63   &   0.00  &   0.00  \\
      2474   &   1.60   &   2.77  &    3.25  &    4.84  &    1.60  &    2.77   &   3.22  &   4.96  \\
      2481   &   0.96   &   2.80  &    5.56  &    6.76  &    0.96  &    2.74   &   5.50  &   6.99  \\
      2545   &   1.00   &   3.07  &    5.79  &    7.59  &    1.00  &    2.93   &   5.70  &   7.73  \\
      2593   &   0.96   &   2.58  &    4.85  &    7.20  &    0.96  &    2.49   &   4.72  &   7.29  \\
      2632   &   1.04   &   2.43  &    4.40  &    5.75  &    1.10  &    2.40   &   4.31  &   5.98  \\
      2640   &   0.87   &   2.18  &    4.26  &    6.28  &    0.90  &    2.09   &   4.16  &   6.37  \\
      2717   &   1.12   &   2.40  &    4.31  &    6.46  &    1.20  &    2.36   &   4.19  &   6.59  \\
      2848   &   1.20   &   2.23  &    4.00  &    5.87  &    1.20  &    2.21   &   3.91  &   6.03  \\
      2938   &   1.12   &   2.28  &    3.93  &    6.73  &    1.12  &    2.23   &   3.80  &   6.64  \\





\hline\hline

\end{longtable}
}


